Bayesian Image Reconstruction using Deep Generative Models

Machine learning models are commonly trained end-to-end and in a supervised setting, using paired (input, output) data. Examples include recent super-resolution methods that train on pairs of (low-resolution, high-resolution) images. However, these end-to-end approaches require re-training every time there is a distribution shift in the inputs (e.g., night images vs daylight) or relevant latent variables (e.g., camera blur or hand motion). In this work, we leverage state-of-the-art (SOTA) generative models (here StyleGAN2) for building powerful image priors, which enable application of Bayes' theorem for many downstream reconstruction tasks. Our method, Bayesian Reconstruction through Generative Models (BRGM), uses a single pre-trained generator model to solve different image restoration tasks, i.e., super-resolution and in-painting, by combining it with different forward corruption models. We keep the weights of the generator model fixed, and reconstruct the image by estimating the Bayesian maximum a-posteriori (MAP) estimate over the input latent vector that generated the reconstructed image. We further use variational inference to approximate the posterior distribution over the latent vectors, from which we sample multiple solutions. We demonstrate BRGM on three large and diverse datasets: (i) 60,000 images from the Flick Faces High Quality dataset (ii) 240,000 chest X-rays from MIMIC III and (iii) a combined collection of 5 brain MRI datasets with 7,329 scans. Across all three datasets and without any dataset-specific hyperparameter tuning, our simple approach yields performance competitive with current task-specific state-of-the-art methods on super-resolution and in-painting, while being more generalisable and without requiring any training. Our source code and pre-trained models are available online: https://razvanmarinescu.github.io/brgm/.

==> Makefile <==
latexRemote:
	scp -r paper.tex 'razvan@sesame.csail.mit.edu:/research/boundaryCrossing/stylegan2/arxiv_paper/'; ssh -Y -t razvan@sesame.csail.mit.edu 'cd /research/boundaryCrossing/stylegan2/arxiv_paper; pdflatex paper.tex'; scp -r 'razvan@sesame.csail.mit.edu:/research/boundaryCrossing/stylegan2/arxiv_paper/paper.pdf' .

latex:
	#step1: increase width of pdflatex log
	#sudo vim /usr/local/texlive/2018/texmf.cnf
	
	#then add

	#max_print_line=1000
	#error_line=254
	#half_error_line=238

	max_print_line=1000 error_line=254 half_error_line=238 texfot pdflatex -shell-escape -interaction nonstopmode -file-line-error paper.tex


# for compressing the images:
compress:
	#find . -name "*.png" | awk '{print substr($1,0,length($1)-4)}' | xargs -n 1 -I {} convert {}.png {}.jpg
	find . -name "*.jpg" | awk '{print substr($1,0,length($1)-4)}' | xargs -n 1 -I {} convert -resize 512x512\> {}.jpg {}.jpg

	 


==> images/Makefile <==
# for teaser: ffhq:0038  xray:0001  brains:0002
N=0002
S=5000
F=$(N)-step$(S)
copy:
	for I in 00598 00599 00600 00601 00602 00603 00604 00605 00606 00607 00608 00609 ; do \
		echo $$I;\
		mkdir -p $(F);\
		scp -r "razvan@thyme.csail.mit.edu:/research/boundaryCrossing/stylegan2/results/$$I*/image$(N)-target.png" . ; mv image$(N)-target.png $(F)/$$I-target.png; \
		scp -r "razvan@thyme.csail.mit.edu:/research/boundaryCrossing/stylegan2/results/$$I*/image$(N)-clean-step$(S).png" . ; mv image$(N)-clean-step$(S).png $(F)/$$I-clean.png;  \
		scp -r "razvan@thyme.csail.mit.edu:/research/boundaryCrossing/stylegan2/results/$$I*/image$(N)-corrupted-step$(S).png" . ; mv image$(N)-corrupted-step$(S).png $(F)/$$I-corrupted.png;  \
		scp -r "razvan@thyme.csail.mit.edu:/research/boundaryCrossing/stylegan2/results/$$I*/image$(N)-true.png" . ; mv image$(N)-true.png $(F)/$$I-true.png;  \
	done

# 


==> tikz-bayesnet/model_citation_influence.tex <==
% model_citation_influence.tex
%
% Copyright (C) 2010,2011 Laura Dietz
% Copyright (C) 2012 Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Citation influence model
% Cite this model as 
% Laura Dietz, Steffen Bickel, Tobias Scheffer. 
% Unsupervised Prediction of Citation Influences. 
% In: Proceedings of International Conference on Machine Learning. 2007

%\beginpgfgraphicnamed{model-citation-influence}
\begin{tikzpicture}

  % Layout the variables
  \matrix[row sep=0.5cm, column sep=1.2cm] (LDA)
  { %
    & %
    & %
    \node[latent] (gamma)  {$\gamma$} ; & %
    \node[latent] (lambda) {$\lambda$} ; & %
    \node[latent] (psi)    {$\psi$} ; %
    \\
    \\
    \node[latent] (theta)  {$\theta$} ; & %
    & %
    \node[latent] (C)      {$C$} ; & %
    \node[latent] (S)      {$S$} ; & %
    \\
    & %
    & %
    \factor       {T-f1}   {Multi} {} {}; & %
    & %
    \factor       {T-f2}   {below:Multi} {} {}; & %
    \\
    \node[latent] (T')     {$T'$} ; & %
    & %
    \node[latent] (T)      {$T$} ; & %
    \\
    \factor       {W'-f}   {Multi} {} {}; & %
    \node[latent] (phi)    {$\phi$} ; & %
    \factor       {W-f}    {Multi} {} {}; %
    \\
    \node[obs] (W')        {$W'$} ; & %
    & %
    \node[obs] (W)         {$W$} ;
    \\
  };

  % Remaining factors
  \factor[above=of T']     {T'-f}     {left:Multi} {} {}; %
  \factor[above=of theta]  {theta-f}  {left:Dir} {} {}; %
  \factor[above=of C]      {C-f}      {left:Multi} {} {}; %
  \factor[above=of S]      {S-f}      {left:Bern} {} {}; %
  \factor[above=of gamma]  {gamma-f}  {left:Dir} {} {}; %
  \factor[above=of lambda] {lambda-f} {left:Beta} {} {}; %
  \factor[above=of psi]    {psi-f}    {left:Dir} {} {}; %
  \factor[above=of phi]    {phi-f}    {left:Dir} {} {}; %

  % Hyperparameters
  \node[const, above=of theta]  (atheta)  {$\alpha_\theta$}; %
  \node[const, above=of phi]    (aphi)    {$\alpha_\phi$}; %
  \node[const, above=of gamma]  (agamma)  {$\alpha_\gamma$}; %
  \node[const, above=of lambda, xshift=-0.5cm] (alambda1)
  {$\alpha_{\lambda_\theta}$}; %
  \node[const, above=of lambda, xshift=0.5cm] (alambda2)
  {$\alpha_{\lambda_\psi}$}; %
  \node[const, above=of psi]    (apsi)    {$\alpha_\psi$}; %

  % Factor connections
  \factoredge {phi}               {W'-f}     {W'} ; %
  \factoredge {phi}               {W-f}      {W} ; %
  \factoredge {theta}             {T'-f}     {T'} ; %
  \factoredge {theta}             {T-f1}     {T} ; %
  \factoredge {psi}               {T-f2}     {T} ; %
  \factoredge {atheta}            {theta-f}  {theta} ; %
  \factoredge {gamma}             {C-f}      {C} ; %
  \factoredge {lambda}            {S-f}      {S} ; %
  \factoredge {agamma}            {gamma-f}  {gamma} ; %
  \factoredge {alambda1,alambda2} {lambda-f} {lambda} ; %
  \factoredge {apsi}              {psi-f}    {psi} ; %
  \factoredge {aphi}              {phi-f}    {phi} ; %

  % Gates
  \gate {W'-gate} {(W'-f)(W'-f-caption)} {T'} ; %
  \gate {W-gate}  {(W-f)(W-f-caption)}   {T} ; %
  \gate {T-gate}  {(T-f1)(T-f1-caption)} {C} ;
  \vgate {T-vgate} %
  {(T-gate)} {$S=0$} %
  {(T-f2)(T-f2-caption)} {$S=1$} %
  {S} ; %

  % Plates
  \plate {LDA1} { %
    (T')(T'-f)(T'-f-caption) %
    (W')(W'-gate) %
  } {$\forall w' \in c$} ; %

  \plate {LDA2} { %
    (LDA1) %
    (theta)(theta-f)(theta-f-caption) %
  } {$\forall c \in \mathcal{C}$} ; %

  \plate {} { %
    (phi)(phi-f)(phi-f-caption) %
  } {$\forall t \in \mathcal{T}$} ; %

  \plate {P1} { %
    (W)(W-gate) %
    (T)(T-vgate) %
    (C)(C-f)(C-f-caption) %
    (S)(S-f)(S-f-caption) %
  } {$\forall w \in d$} ;

  \plate {} { %
    (P1) %
    (gamma)(gamma-f)(gamma-f-caption) %
    (lambda)(lambda-f)(lambda-f-caption) %
    (psi)(psi-f)(psi-f-caption) %
  } {$\forall d \in \mathcal{D}$} ; %

\end{tikzpicture}
%\endpgfgraphicnamed

%%% Local Variables: 
%%% mode: tex-pdf
%%% TeX-master: "example"
%%% End: 


==> tikz-bayesnet/model_lda.tex <==
% model_lda.tex
%
% Copyright (C) 2010,2011 Laura Dietz
% Copyright (C) 2012 Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Latent Diriclet allocation model

%\beginpgfgraphicnamed{model-lda}
\begin{tikzpicture}[x=1.7cm,y=1.8cm]

  % Nodes

  \node[obs]                   (X)      {$X$} ; %
  \node[latent, above=of X]    (T)      {$T$} ; %
  \node[latent, above=of T]    (theta)  {$\theta$}; %
  \node[const, above=of theta] (atheta) {$\alpha_\theta$};


  % Factors
  \factor[above=of X]     {X-f}     {Multi} {} {} ; %
  \factor[above=of T]     {T-f}     {left:Multi} {} {} ; %
  \factor[above=of theta] {theta-f} {left:Dir} {} {} ; %

  % More nodes
  \node[latent, right=of X-f] (phi)  {$\phi$}; %
  \node[const, above=of phi]  (aphi) {$\alpha_\phi$}; %

  \factor[above=of phi] {phi-f} {right:Dir} {} {} ; %

  \factoredge {theta}  {T-f}     {T} ; %
  \factoredge {atheta} {theta-f} {theta} ; %
  \factoredge {phi}    {X-f}     {X} ; %
  \factoredge {aphi}   {phi-f}   {phi} ; %

  \gate {X-gate} {(X-f)(X-f-caption)} {T}

  \plate {plate1} { %
    (X)(X-gate) %
    (T)(T-f)(T-f-caption) %
  } {$\forall 1 \leq i \leq n_d$}; %
  \plate {} { %
    (plate1) %
    (theta)(theta-f)(theta-f-caption) %
  } {$\forall d \in \mathcal{D}$} ; %
  \plate {} { %
    (phi)(phi-f)(phi-f-caption) %
  } {$\forall t \in \mathcal{T}$} ; %

\end{tikzpicture}
%\endpgfgraphicnamed

%%% Local Variables: 
%%% mode: tex-pdf
%%% TeX-master: "example"
%%% End: 


==> tikz-bayesnet/model_pca.tex <==
% model_pca.tex
%
% Copyright (C) 2012 Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% PCA model

%\beginpgfgraphicnamed{model-pca}
\begin{tikzpicture}

  % Define nodes
  \node[obs]                               (y) {$y$};
  \node[latent, above=of y, xshift=-1.2cm] (w) {$\mathbf{w}$};
  \node[latent, above=of y, xshift=1.2cm]  (x) {$\mathbf{x}$};
  \node[latent, right=2cm of y]            (t) {$\tau$};

  % Connect the nodes
  \edge {x,w,t} {y} ; %

  % Plates
  \plate {yx} {(x)(y)} {$N$} ;
  \plate {} {(w)(y)(yx.north west)(yx.south west)} {$M$} ;

\end{tikzpicture}
%\endpgfgraphicnamed

%%% Local Variables: 
%%% mode: tex-pdf
%%% TeX-master: "example"
%%% End: 


==> tikz-bayesnet/model_pca2.tex <==
% model_pca2.tex
%
% Copyright (C) 2010,2011 Laura Dietz
% Copyright (C) 2012 Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% PCA model

%\beginpgfgraphicnamed{model-pca}
\begin{tikzpicture}

  % Define nodes

  % Y
  \node[obs]          (y)   {$y$}; %
  \factor[above=of y] {y-f} {left:$\mathcal{N}$} {} {} ; %

  % W and X
  \node[det, above=of y]            (dot) {dot} ; % 
  \node[latent, above left=1.2 of dot]  (w)   {$\mathbf{w}$}; %
  \node[latent, above right=1.2 of dot] (x)   {$\mathbf{x}$}; %

  % W hyperparameters
  \node[const, above=1.2 of w, xshift=-0.5cm] (mw) {$\mu_w$} ; %
  \node[const, above=1.2 of w, xshift=0.5cm]  (aw) {$\alpha_w$} ; %

  % X hyperparameters
  \node[const, above=1.2 of x, xshift=-0.5cm] (mx) {$\mu_x$} ; %
  \node[const, above=1.2 of x, xshift=0.5cm]  (ax) {$\alpha_x$} ; %

  % noise
  \node[latent, right=2.5cm of y-f]         (t)   {$\tau$}; %
  \node[const, above=of t, xshift=-0.5cm] (at)  {$\alpha_\tau$} ; %
  \node[const, above=of t, xshift=0.5cm]  (bt)  {$\beta_\tau$} ; %

  % Factors
  \factor[above=of w] {w-f} {left:$\mathcal{N}$} {mw,aw} {w} ; %
  \factor[above=of x] {x-f} {left:$\mathcal{N}$} {mx,ax} {x} ; %
  \factor[above=of t] {t-f} {left:$\mathcal{G}$} {at,bt} {t} ; %
  \factoredge {dot,t} {y-f} {y} ; %

  % Connect w and x to the dot node
  \edge[-] {w,x} {dot} ;

  % Plates
  \plate {yx} { %
    (y)(y-f)(y-f-caption) %
    (x)(x-f)(x-f-caption) %
    (dot) %
  } {$N$} ;
  \plate {} {%
    (y)(y-f)(y-f-caption) %
    (w)(w-f)(w-f-caption) %
    (dot) %
    (yx.north west)(yx.south west) %
  } {$M$} ;

\end{tikzpicture}
%\endpgfgraphicnamed

%%% Local Variables: 
%%% mode: tex-pdf
%%% TeX-master: "example"
%%% End: 



==> tikz-bayesnet/tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

